Into the Unknown Unknowns: Engaged Human Learning through Participation in Language Model Agent Conversations

While language model (LM)-powered chatbots and generative search engines excel at answering concrete queries, discovering information in the terrain of unknown unknowns remains challenging for users. To emulate the common educational scenario where children/students learn by listening to and participating in conversations of their parents/teachers, we create Collaborative STORM (Co-STORM). Unlike QA systems that require users to ask all the questions, Co-STORM lets users observe and occasionally steer the discourse among several LM agents. The agents ask questions on the user's behalf, allowing the user to discover unknown unknowns serendipitously. To facilitate user interaction, Co-STORM assists users in tracking the discourse by organizing the uncovered information into a dynamic mind map, ultimately generating a comprehensive report as takeaways. For automatic evaluation, we construct the WildSeek dataset by collecting real information-seeking records with user goals. Co-STORM outperforms baseline methods on both discourse trace and report quality. In a further human evaluation, 70% of participants prefer Co-STORM over a search engine, and 78% favor it over a RAG chatbot.

==> examples/discourse_snippet3.tex <==
\begin{showcase}[title=Topic: AlphaFold 3]

{Previous discourse focuses on Background, Technical Aspects covering accessibility enhancement for researches and advancements in biomelecular structure prediction, as well as impact and applications in biotechnology applications.}

|\userbg{User:}|
Any impact on the stock market?

|\expertbg{General Knowledge Provider:}|
{More content omitted} It stands to greatly benefit pharmaceutical giants like Pfizer, Merck, and Novartis, as well as smaller biotech firms like Schrödinger and Exscientia[21][32][66][67][68][69][70][71][72]. These advancements might not move the market immediately, but they could significantly boost the stock performance of companies that leverage this tech. So, keeping an eye on how these firms integrate AlphaFold 3 could be key to understanding its broader market implications.

|\expertbg{General Knowledge Provider:}|
{More content omitted} The biotech sector has shown resilience, even during economic downturns, thanks to continuous innovation and the successful transition of assets to clinical phases [74]. Government support and rapid tech adoption have further bolstered this sector [77]. A notable example is BioNTech, whose collaboration with Pfizer on the Covid-19 vaccine significantly boosted its market value [78].

{rest of discourse omitted}

\end{showcase}
